A Data-Efficient Approach for Long-Term Human Motion Prediction Using Maps of Dynamics

Human motion prediction is essential for the safe and smooth operation of mobile service robots and intelligent vehicles around people. Commonly used neural network-based approaches often require large amounts of complete trajectories to represent motion dynamics in complex semantically-rich spaces. This requirement may complicate deployment of physical systems in new environments, especially when the data is being collected online from onboard sensors. In this paper we explore a data-efficient alternative using maps of dynamics (MoD) to represent place-dependent multi-modal spatial motion patterns, learned from prior observations. Our approach can perform efficient human motion prediction in the long-term perspective of up to 60 seconds. We quantitatively evaluate its accuracy with limited amount of training data in comparison to an LSTM-based baseline, and qualitatively show that the predicted trajectories reflect the natural semantic properties of the environment, e.g. the locations of short- and long-term goals, navigation in narrow passages, around obstacles, etc.

==> related_work.tex <==
\section{RELATED WORK} \label{section-relatedwork}

Human motion prediction has been studied extensively in recent years. With different prediction horizons, the human motion prediction problem can be divided into short-term (1--\SI{2}{\second}), long-term (up to \SI{20}{\second}) \cite{rudenko2020human}, and very long-term (which we define as over \SI{20}{\second}). Several approaches address long-term motion prediction, e.g. full-body motion \cite{tanke2021intention} or in the context of vehicle routing and GPS positioning \cite{cheng2010geodtn,xiao2018goi}, but, to the best of our knowledge, very long-term prediction of dense navigation trajectories has not been addressed before.

One approach to predict long-term human motion is to account for various semantic attributes of the static environment. For instance, prior knowledge of potential goals in the environment can be used in planning-based methods. \textcite{ziebart2009planning,karasev2016intent} propose planning MDP-based approaches for long-term goal-directed global motion prediction. \textcite{Rudenko2018iros} extends this line of work by accounting for local social interactions, which is shown to outperform prior art in the long-term map-aware perspective. %There are several approaches that estimate goals to achieve long-term prediction. \textcite{ikeda2013modeling} propose to learn sub-goals, i.e., way-points that pedestrians have the tendency to pass before reaching the final destination, and model the long-term behavior of pedestrians with transition probabilities between sub-goals. Information about interaction with objects in the environment can also be used to predict the navigation goal of a moving human. \textcite{bruckschen2019human} propose to learn a transition model of sequential object interactions and use it to infer the navigation goal using a recursive Bayes' filter.

Another popular approach to make long-term predictions is using clustering to represent observed long-term motion patterns, e.g., using expectation-maximization~\cite{bennewitz2005learning}. \textcite{chen2008pedestrian} use constrained gravitational clustering 
%(CGC) 
for dynamically grouping the observed trajectories, learning also how motion patterns change over time. \textcite{bera2016glmp} learn global and local motion patterns using Bayesian inference in real-time. One shortcoming of clustering-based methods is that they depend on complete trajectories as input. In many cases, e.g. in cluttered environments or from a first-person perspective \cite{dondrup2015tracker}, it is difficult to observe long trajectories, or cluster shorter tracklets and incomplete trajectories in a meaningful way.

These clustering-based methods are non-sequential and directly model the distribution over full trajectories. In contrast to that, transition-based approaches \cite{thompson2009probabilistic, wang2015modeling, ballan2016knowledge, kucner2013conditional, Jari2012iMac} describe human motion with causally conditional models over time, generating sequential predictions by learning local motion patterns.

%\textcite{wang2015modeling} propose an approach to modeling human motion dynamics by capturing both local spatiotemporal correlations and implicit long-term dependencies with a grid-based representation. This approach builds a multi-scale conditional transition map and treats human dynamics as a change of occupancy in grid map cells. 

Further, there are physics-based approaches that build a kinematic model without considering other forces that govern the motion. The constant velocity model (CVM) is a simple yet potent approach to predict human motion. \textcite{scholler2019simpler} has shown CVM to outperform several state-of-the-art neural predictors at the \SI{4.8}{\second} prediction horizon. On the other hand, CVM is not reliable for long-term prediction as it ignores all environment information.

Finally, many neural network approaches for motion prediction have been presented in recent years, based on LSTMs \cite{alahi2016social}, GANs \cite{sadeghian2018sophie}, CNNs \cite{mohamed2020social}, CVAEs \cite{salzmann2020trajectronpp} and transformers \cite{giuliari2021transformer}. Most of these approaches focus on learning to predict stochastic interactions between diverse moving agents in the short-term perspective in scenarios where the effect of the environment topology and semantics is minimal. Our approach, on the other hand, targets specifically the long-term perspective, where the environment effects become critical for making accurate predictions.

Our approach to motion prediction leverages maps of dynamics (MoDs), which encode motion as a feature of the environment by building spatio-temporal models of the patterns followed by dynamic objects (such as humans) in the environment \cite{kucner2020probabilistic}. There are several approaches for building maps of dynamics from observed motion. Some MoDs represent human dynamics in occupancy grid maps~\cite{wang2015modeling}. Another type of MoDs clusters human trajectories as mentioned above \cite{bennewitz2005learning}. \textcite{chen2016augmented} present an approach that uses a dictionary learning algorithm to develop a part-based trajectory representation. 
%In trajectory modeling, this 
%This approach does not consider velocity and only models heading.

None of the above approaches encode the velocity of motion in the map of dynamics; only the direction.
%
However, MoDs can also be based on mapping velocity observations into flow models, which has the  distinct advantage that the MoD can be built from incomplete or spatially sparse data. 
An example of this class of MoDs is the probabilistic Circular-Linear Flow Field map (CLiFF-map)~\cite{kucner2017enabling} that we use in this paper. CLiFF-map uses a Gaussian mixture model (GMM) to describe multimodal flow patterns at each location. In this paper, we use sampled directions from the CLiFF map to predict stochastic long-term human motion.
%, which is the key feature to predict stochastic long-term human motion. In contrast to MoDs that map trajectories, CLiFF-map allows building maps of motion patterns from incomplete or spatially sparse data.

%Andrey: I removed this passage to save some space, it does not seem to add critical information to the method presented in this particular paper
%When building flow models, temporal information can also be incorporated. \textcite{molina2018modelling} apply the Frequency Map Enhancement (FreMEn \cite{krajnik2017fremen}), which is a model describing spatiotemporal dynamics in the frequency domain, to build a time-dependent probabilistic map to model periodic changes in people flow. The human motion orientation is discretized. Another method of incorporating temporal information is proposed by \textcite{zhi2019spatiotemporal}. Their approach uses a long-short term memory (LSTM) network \cite{hochreiter1997lstm} to provide a multimodal probability distribution of movement directions of a typical object in the environment over time.

Closest to our method is the approach by \textcite{BARATA2021107631}.
%This approach is in the field of computer vision.
In their work, a vector field that represents the most common direction at each point is constructed and human trajectories are predicted by inferring the most probable sequence through the vector field.
%The motion field is constructed with a number of motion vectors. 
While our approach uses a probabilistic MoD that represents speed and orientation jointly with a multimodal distribution in each location, in \textcite{BARATA2021107631}, the motion distribution is unimodal and speed is not modeled, only orientation. The evaluation in~\textcite{BARATA2021107631} assumes a fixed prediction horizon of \SI{4.8}{\second}, 
%whereas we show our approach to estimate human motion well for up to \SI{50}{\second}.
whereas we show our approach to estimate human motion more accurately than the state of the art for up to \SI{50}{\second}.
%whereas we show our approach to accurately estimate human motion for up to \SI{50}{\second}.

%While the aforementioned prediction approaches aim for long-term human motion prediction whose prediction horizons are mostly less than 10~s, in this work, for the first time, we focus on very long-term human motion predictions up to 50~s. Our approach exploits MoDs to predict human motions. The approach can be applied with several MoDs that represent velocities. In the present approach, we choose to use the CLiFF-map because it can preserve multimodal nature of people flow and has a continuous representation of orientations. We predict trajectories using sampling motions from the MoD over a simple constant velocity model, as detailed in the next section.


% Closest to our method is the approach proposed by Chen et al. \cite{chen2016augmented}, which combines merits of Markovian-based and clustering-based approaches. In the work, a dictionary learning algorithm is proposed for developing a part-based trajectory representation. The trajectory is represented using vector of velocity and the binary activeness variable which specified whether the trajectory goes through a particular gird. The method corresponds the learned dictionary atoms to local motion patterns, and develops  an augmented semi-nonnegative sparse coding algorithm for solving the dictionary learning problem.

% sparse map, dense map

% CLiFF-map can be used to model the flow of discrete objects (e.g. people, vehicles or other robots) as well as continuous media (e.g. air). Moreover, CLiFF-map also contains information about how much a region in the environment has been observed and how much motion there is. The CLiFF-map allows us to generate plans based on the learned flow patterns for the entire map and not only for regions where the robot can currently observe motion.

==> results.tex <==
\section{RESULTS} \label{section-results}

% In the ATC dataset (see \cref{fig:atc_final}), both our approach and IS-MDP outperform the CVM method. One benefit of our approach is that it handles goals implicitly. In the IS-MDP method, explicit goals are required and its performance strongly depends on it. Our approach performs better than the IS-MDP method because it manages both the short- and long-term goals implicitly. 

%In short-term prediction, all approaches perform on par :)
%Given the standard deviation, especially. It is higher in THÖR1, so the results strongly depend on the specific piece of GT data

%In short-term predictions, given the variance in the ground truth trajectories, all approaches perform on par.
In this section, we present experimental results obtained with our approach and baselines in ATC and THÖR datasets. The performance evaluation is conducted using both quantitative and qualitative analysis, and we further investigate the approach's performance through a parameter analysis.

\subsection{Quantitative Results}
\cref{fig:atc_final,fig:thor_final} show the quantitative results obtained in the ATC and THÖR datasets. We compare our CLiFF-LHMP approach with IS-MDP~\cite{Rudenko2018iros} and CVM. In the short-term perspective all approaches perform on par. The mean ADE is marginally lower for CVM compared to the other predictors below \SI{6}{\second} in ATC, below \SI{10}{\second} in THÖR1, and below \SI{4}{\second} in THÖR3. In THÖR3 there are more obstacles that people need to avoid, while THÖR1 and ATC include more open spaces. In open spaces without obstacles, a constant velocity prediction is often the optimal predictor in the short-term perspective \cite{rudenko2022atlas}. In comparison, our approach also accounts for possible deviations from the straight trajectories which increases the ADE slightly.
For prediction horizons less than \SI{10}{\second}, IS-MDP performs better than CLiFF-LHMP. However, the IS-MDP method requires additional input (goal points and the obstacle map) and its performance strongly depends on both. In contrast, our approach makes predictions without explicit knowledge about goals and implicitly accounts for the obstacle layout, as well as the specific ways people navigate in the environment.

In long-term predictions above \SI{10}{\second}, both CLiFF-LHMP and IS-MDP outperform the CVM method. Our approach is substantially better than IS-MDP when the prediction horizon is above \SI{20}{\second} due to exploiting location-specific motion patterns implicitly, thus overcoming a known limitation of the MDP-based methods \cite{Rudenko2018iros}. \cref{tab:expres} summarises the performance results of our method against the baseline approaches at the maximum prediction horizon. CLiFF-LHMP approach accurately predict human motion up to \SI{50}{\second} within \SI{5}{\metre} mean ADE. At \SI{50}{\second} in the ATC dataset, our method achieves a 45\% ADE and 55\% FDE improvement in performance compared to IS-MDP. At \SI{12}{\second} in THÖR1 and THÖR3, our method achieves an improvement of 6.3\% and 13.3\% ADE (25.7\%, 27.8\% FDE), respectively.

\cref{fig:atc_final,fig:thor_final} also show that the standard deviation of ADE and FDE is generally lower in the CLiFF-LHMP results, compared to CVM and IS-MDP. This indicates that our approach makes more consistent predictions, both in the short- and long-term perspective.

\begin{table}[t]
    \centering
    \begin{tabular}{lllll}
     \toprule
        \textbf{Dataset} & \textbf{Horizon} & \multicolumn{3}{c}{\textbf{ADE/FDE} (m)} \\
          & & CLiFF-LHMP & IS-MDP & CVM \\
        \midrule
        ATC & 50 \si{\second} & \textbf{4.6} / \textbf{9.6} & 8.4 / 21.3 & 12.4 / 27.1 \\
        THÖR1 & 12 \si{\second} & \textbf{1.5} / \textbf{2.6} & 1.6 / 3.5 & 1.8 / 3.8 \\
        THÖR3 & 12 \si{\second} & \textbf{1.3} / \textbf{2.6} & 1.5 / 3.6 & 2.8 / 6.1 \\
        \bottomrule
    \end{tabular}
    \caption{Long-term prediction horizon results on different datasets}
    \label{tab:expres}
\vspace*{-5mm}
\end{table}


\begin{figure}
\centering
%.471, .45
\includegraphics[width=.50\linewidth]{figures/ATC_baseline_compare_ADE.pdf}
\includegraphics[width=.48\linewidth]{figures/ATC_baseline_compare_FDE.pdf}
%\includegraphics[width=.45\linewidth]{figures/atc_res_ADE.pdf}
%\includegraphics[width=.45\linewidth]{figures/atc_res_FDE.pdf}
\caption{ADE/FDE (mean $\pm$ one std. dev.) in the ATC dataset with prediction horizon 1--\SI{50}{\second}.}
\label{fig:atc_final}
\vspace*{-5mm}
\end{figure}

\begin{figure}[t]
\centering
%.47, .45
\includegraphics[width=.47\linewidth]{figures/thor1_baseline_compare_ADE2.pdf}
\includegraphics[width=.45\linewidth]{figures/thor1_baseline_compare_FDE2.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor3_baseline_compare_ADE2.pdf}
\includegraphics[width=.47\linewidth]{figures/thor3_baseline_compare_ADE_new.pdf}
\includegraphics[width=.455\linewidth]{figures/thor3_baseline_compare_FDE2.pdf}
\caption{ADE/FDE (mean $\pm$ one std. dev.) in the THÖR1 \textbf{(top)} and THÖR3 \textbf{(bottom)} dataset with prediction horizon 0.4--\SI{12}{\second}.}
\label{fig:thor_final}
\vspace*{-5mm}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=.3\linewidth]{figures/rs_123_FDE_ADE.pdf}
%\includegraphics[width=.3\linewidth]{figures/beta_01110_ADE.pdf}
%\includegraphics[width=.3\linewidth]{figures/rs_123_ADE.pdf}
%\includegraphics[width=.3\linewidth]{figures/obs_358_FDE.pdf}
%\includegraphics[width=.3\linewidth]{figures/beta_01110_FDE.pdf}
%\includegraphics[width=.3\linewidth]{figures/rs_123_FDE.pdf}
%\caption{ADE/FDE in the ATC dataset different parameters.}
%\label{fig:parameter-eva}
%\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=.3235\linewidth]{figures/resub/obs_358_ADE_new.pdf}
\includegraphics[width=.3235\linewidth]{figures/resub/beta_05110_ADE_new.pdf}
\includegraphics[width=.315\linewidth]{figures/resub/rs_123_ADE_bottom_new.pdf}
%\includegraphics[width=1\linewidth]{figures/obs_358_ADE.pdf}
%\includegraphics[width=1\linewidth]{figures/beta_05110_ADE.pdf}
%\includegraphics[width=1\linewidth]{figures/rs_123_ADE_bottom.pdf}
\caption{%ADE/FDE in the ATC dataset different parameters: 
Parameter analysis on the ATC dataset, showing the ADE (mean $\pm$ one std. dev.) over different prediction horizons vs the 
observation horizon $O_s$ \textbf{(left)}, kernel parameter $\beta$ \textbf{(middle)} and sampling radius $r_s$ \textbf{(right)}.}
\label{fig:parameter-eva}
\vspace*{-6mm}
\end{figure*}

\subsection{Parameter Analysis}
In the experiments with different observation horizons (see \cref{fig:parameter-eva}, left), our method performs robustly when the observation horizon is as low as \SI{1.2}{\second}. In the experiments with different $\beta$ values (see \cref{fig:parameter-eva}, middle), we find that $\beta = 1$ is a good trade-off. Lower $\beta$ values make the predictor trust the CLiFF-map more, which can lead to jumps between distinct motion patterns. Setting $\beta$ to a high value such as 10 slightly improves the performance, however
%at the cost of a considerably reduced number of successfully predicted trajectories.
the predictor is prone to failure in the long-term perspective, sharing this drawback with the CVM model.
The reason is that we stop predicting when the CLiFF-map is not any longer available close to the predicted  location. So, if more trust is put on the CVM component, many ground truth trajectories cannot be predicted successfully with in the long term. When the planning horizon is set to \SI{50}{\second}, 84\% of ground truth trajectories can be predicted successfully with $\beta = 1$, while with $\beta = 10$, the ratio drops to 52.3\%. Also when the prediction is dominated by CVM component, the top k-ADE/FDE scores are worse due to the reduced diversity of the predictions.

In the experiments with different values of the sampling radius $r_s$ (see \cref{fig:parameter-eva}, right), we observe a stable prediction performance. Therefore, it is reasonable to set $r_s = 1$ in order to reduce the computation cost. 

%Our method predict robustly for different prediction time step
In our experiments with the prediction time step $\Delta t$, we observe robust performance with slight improvement when making higher frequency predictions ($\Delta t=$\SI{0.4}{\second} vs. \SI{1.0}{\second}, see \cref{fig:thor_delta_t}). Smaller $\Delta t$ is recommended in cluttered environments, such as THÖR dataset. Making iterative predictions with a smaller time step naturally comes at the expense of computational cost increasing linearly for CLiFF-LHMP.
%In the experiments varying $\Delta t$ in THÖR, we find that our approach is not very sensitive to $\Delta t$ over the range of values we investigated (see \cref{fig:thor_delta_t}).
Selecting a larger prediction time step $\Delta t=$\SI{1.0}{\second} drops the performance in THÖR by only approx. 5\% at the maximum prediction horizon, as compared to $\Delta t=$\SI{0.4}{\second}.

%When use the same prediction step in THÖR dataset as in ATC dataset, We only see a minor deterioration of around 5\%, 

%In the experiments with the prediction time step $\Delta t$ in the cluttered THÖR dataset, our method is robust to coarse predictions (see \cref{fig:thor_delta_t}). For instance, selecting a higher prediction step value (\SI{1.0}{\second}) will decrease the performance by around 5\% at the maximum prediction horizon.






\subsection{Qualitative Results}
\Cref{fig:atc_predict_example,fig:thor_predict_example} show qualitative results with example predictions. Our approach correctly captures the motion patterns in each scenario, utilizing the environment information during the prediction. \Cref{fig:thor_predict_example} shows that the predicted trajectories avoid the obstacles, even though an obstacle map is not used for predictions. Furthermore, using maps of dynamics built from the observations of human motion makes it possible to predict motion through regions which appear as obstacles in an occupancy map, for example across stairs and through narrow passages (see~\cref{fig:atc_predict_example}). Similarly, aiding prediction with the MoD input focuses the results towards more intensively used areas of the environment, avoiding semantically-insignificant and empty regions, e.g. corners of the room (see~\cref{fig:thor_predict_example}).

%\begin{figure}
%\centering
%\includegraphics[width=.47\linewidth]{figures/resub/thor1_cvm_vs_mod.pdf}
%\includegraphics[width=.47\linewidth]{figures/resub/thor3_cvm_vs_mod.pdf}
%\caption{Ratio of collided predicted trajectories and total trajectories in the THÖR1 \textbf{(left)} and THÖR3 \textbf{(right)} dataset with planning horizon 0.4--\SI{12}{\second}.}
%\label{fig:thor_collide}
%\vspace*{-1mm}
%\end{figure}

\begin{figure}
\centering
\includegraphics[width=.47\linewidth]{figures/resub/thor1_delta_t_ADE.pdf}
\includegraphics[width=.47\linewidth]{figures/resub/thor3_delta_t_ADE.pdf}
%\includegraphics[width=.47\linewidth]{figures/resub/thor1_delta_t.pdf}
%\includegraphics[width=.47\linewidth]{figures/resub/thor3_delta_t.pdf}

\caption{Prediction time step $\Delta t$ analysis on THÖR1 \textbf{(left)} and THÖR3 \textbf{(right)} datasets, showing the ADE (mean $\pm$ one std. dev.) over different prediction horizons.}
\label{fig:thor_delta_t}
\vspace*{-3mm}
\end{figure}

\begin{figure*}
\centering
%\includegraphics[width=.4\linewidth]{figures/predict_example1.pdf}%
%\includegraphics[width=.4\linewidth]{figures/predict_example2.pdf}\\
%\includegraphics[width=.4\linewidth]{figures/predict_example3.pdf}%
%\includegraphics[width=.4\linewidth]{figures/predict_example4.pdf}
\includegraphics[clip,trim=0mm 15mm 0mm 0mm,height=40mm]{figures/predict_example1.pdf}%
\includegraphics[clip,trim=21mm 15mm 0mm 0mm,height=40mm]{figures/predict_example2.pdf}\\
\includegraphics[clip,trim=0mm  0mm 0mm 0mm,height=45mm]{figures/predict_example3.pdf}%
\includegraphics[clip,trim=21mm 0mm 0mm 0mm,height=45mm]{figures/predict_example4.pdf}
\caption{Predictions in ATC with $T_s=50$ \SI{}{\second}. \textbf{Red} lines show ground truth trajectories. \textbf{Green} dots show the observed states and \textbf{blue} dots show the predicted states (more transparent for later time steps).
  Note that %the true trajectory is close to at least one prediction in all cases %,  predictions are plausible,  and that
  we  correctly predict trajectories crossing obstacles such as stairs (top of the map) and exits (left of the map).
}
\label{fig:atc_predict_example}
\vspace*{-5mm}
\end{figure*}

\begin{figure}
\centering
%\includegraphics[height=.45\linewidth]{figures/thor1_predict_example1.pdf}%
%\includegraphics[height=.45\linewidth]{figures/thor1_predict_example2.pdf}\\
%\includegraphics[height=.45\linewidth]{figures/thor3_predict_example1.pdf}%
%\includegraphics[height=.45\linewidth]{figures/thor3_predict_example2.pdf}

%\includegraphics[clip,trim=  0mm 16mm 0mm 0mm,height=35.5mm]{figures/thor1_predict_example1.pdf}%
%\includegraphics[clip,trim= 22mm 16mm 0mm 0mm,height=35.5mm]{figures/thor1_predict_example2.pdf}\\
%\includegraphics[clip,trim=  0mm  0mm 0mm 0mm,height=39mm]{figures/thor3_predict_example1.pdf}%
%\includegraphics[clip,trim= 22mm  0mm 0mm 0mm,height=39mm]{figures/thor3_predict_example2.pdf}

\includegraphics[clip,trim=  0mm 15mm 0mm 0mm,height=35.5mm]{figures/thor1_predict_example1.pdf}%
\includegraphics[clip,trim= 22mm 15mm 0mm 0mm,height=35.5mm]{figures/thor1_predict_example2.pdf}\\
\includegraphics[clip,trim=  0mm  0mm 0mm 0mm,height=39mm]{figures/thor3_predict_example1.pdf}%
\includegraphics[clip,trim= 22mm  0mm 0mm 0mm,height=39mm]{figures/thor3_predict_example2.pdf}
\caption{Predictions in THÖR1 \textbf{(top)} and THÖR3 \textbf{(bottom)} with $T_s=12$~s. \textbf{Red} line shows the ground truth trajectory. \textbf{Green} dots show the observed states and \textbf{blue} dots show the predicted future states, shown more transparent for later time instances.}
\label{fig:thor_predict_example}
\vspace*{-5mm}
\end{figure}


%\begin{figure}
%\centering
%.47, .45
%\includegraphics[width=.470\linewidth]{figures/thor1_baseline_compare_ADE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor1_baseline_compare_FDE.pdf}
%\includegraphics[width=.470\linewidth]{figures/thor1_res_ADE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor1_res_FDE.pdf}
%\caption{ADE/FDE in the THÖR1 dataset with planning horizon 0.4--12~s.}
%\label{fig:thor1_final}
%\end{figure}


%\begin{figure}
%\centering
% .45, .462
%\includegraphics[width=.45\linewidth]{figures/thor3_baseline_compare_ADE.pdf}
%\includegraphics[width=.462\linewidth]{figures/thor3_baseline_compare_FDE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor3_res_ADE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor3_res_FDE.pdf}
%\caption{ADE/FDE in the THÖR3 dataset with planning horizon 0.4--12~s.}
%\label{fig:thor3_final}
%\end{figure}

%\begin{figure}
%\centering
% .45, .462
%\includegraphics[width=.45\linewidth]{figures/thor3_baseline_compare_ADE.pdf}
%\includegraphics[width=.462\linewidth]{figures/thor3_baseline_compare_FDE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor3_res_ADE.pdf}
%\includegraphics[width=.45\linewidth]{figures/thor3_res_FDE.pdf}
%\caption{ADE/FDE in the THÖR3 dataset with planning horizon 0.4--12~s.}
%\label{fig:thor3_final}
%\end{figure}

%\begin{figure}
%\centering
% .45, .4697
%\includegraphics[width=.10\linewidth]{figures/obs_358_ADE.pdf}
%\includegraphics[width=.1\linewidth]{figures/obs_358_FDE.pdf}
%\caption{ADE/FDE in the ATC dataset with observation horizon is 1.2 s, 2 s, 3.2 s.}
%\label{fig:atc_obs_358}
%\end{figure}

%\begin{figure}
%\centering
% .45, .45
%\includegraphics[width=.1\linewidth]{figures/beta_01110_ADE.pdf}
%\includegraphics[width=.1\linewidth]{figures/beta_01110_FDE.pdf}

%\caption{ADE/FDE in the ATC dataset with $\beta$ is 0.5, 1, 10. With higher $\beta$ value, the degree of impact brought by MoD is lower, then the approach is closer to CVM.}
%\label{fig:atc_beta_05110}
%\end{figure}

%\begin{figure}
%\centering
%.45, .4843
%\includegraphics[width=.1\linewidth]{figures/rs_123_ADE.pdf}
%\includegraphics[width=.1\linewidth]{figures/rs_123_FDE.pdf}
%\caption{ADE/FDE in the ATC dataset with $r_s$ is 1~m, 2~m, 3~m.}
%\label{fig:atc_rs_123}
%\end{figure}




